Using Machine Learning to Compute Constrained Optimal Carbon Tax Rules

We develop a computational framework for deriving Pareto-improving and constrained optimal carbon tax rules in a stochastic overlapping generations (OLG) model with climate change. By integrating Deep Equilibrium Networks for fast policy evaluation and Gaussian process surrogate modeling with Bayesian active learning, the framework systematically locates optimal carbon tax schedules for heterogeneous agents exposed to climate risk. We apply our method to a 12-period OLG model in which exogenous shocks affect the carbon intensity of energy production, as well as the damage function. Constrained optimal carbon taxes consist of tax rates that are simple functions of observables and revenue-sharing rules that guarantee that the introduction of the taxes is Pareto improving. This reveals that a straightforward policy is highly effective: a Pareto-improving linear tax on cumulative emissions alone yields a 0.42% aggregate welfare gain in consumption-equivalent terms while adding further complexity to the tax provides only a marginal increase to 0.45%. The application demonstrates that the proposed approach produces scalable tools for macro-policy design in complex stochastic settings. Beyond climate economics, the framework offers a template for systematically analyzing welfare-improving policies in various heterogeneous-agent problems.

==> figures/lin_S/sim_ee_discrepancies_lin_S_only_pareto.tex <==
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
& Gen 1 & Gen 2 & Gen 3 & Gen 4 & Gen 5 & Gen 6 & Gen 7 & Gen 8 & Gen 9 & Gen 10 & Gen 11 \\
\midrule
Rel EE Mean          & 0.0003 & 0.0003 & 0.0004 & 0.0011 & 0.0020 & 0.0023 & 0.0021 & 0.0012 & 0.0005 & 0.0004 & 0.0006 \\
Rel EE 99.9     & 0.0014 & 0.0022 & 0.0017 & 0.0018 & 0.0032 & 0.0037 & 0.0032 & 0.0025 & 0.0014 & 0.0014 & 0.0017 \\
Rel Value Function Mean       & 0.0004 & 0.0003 & 0.0003 & 0.0004 & 0.0004 & 0.0010 & 0.0006 & 0.0007 & 0.0002 & 0.0003 & 0.0008 \\
Rel Value Function 99.9  & 0.0021 & 0.0021 & 0.0021 & 0.0023 & 0.0021 & 0.0028 & 0.0024 & 0.0022 & 0.0020 & 0.0021 & 0.0028 \\
\bottomrule
\end{tabular}

==> figures/linear_transfers/simulated_euler_disc_latex.tex <==

\begin{tabular}{@{}lccccccccccc@{}}
\toprule
& Gen 1 & Gen 2 & Gen 3 & Gen 4 & Gen 5 & Gen 6 & Gen 7 & Gen 8 & Gen 9 & Gen 10 & Gen 11 \\
\midrule
Rel EE Mean          & 0.0004 & 0.0003 & 0.0005 & 0.0004 & 0.0005 & 0.0004 & 0.0004 & 0.0005 & 0.0010 & 0.0011 & 0.0007 \\
Rel EE 99.9     & 0.0033 & 0.0019 & 0.0029 & 0.0018 & 0.0031 & 0.0024 & 0.0021 & 0.0019 & 0.0037 & 0.0041 & 0.0034 \\
Rel Value Function Mean       & 0.0004 & 0.0002 & 0.0002 & 0.0003 & 0.0004 & 0.0003 & 0.0002 & 0.0005 & 0.0005 & 0.0006 & 0.0006 \\
Rel Value Function 99.9  & 0.0015 & 0.0015 & 0.0017 & 0.0018 & 0.0015 & 0.0013 & 0.0011 & 0.0018 & 0.0020 & 0.0026 & 0.0021 \\
\bottomrule
\end{tabular}
